Sums of Uncertainty: Refinements Go Gradual

A long-standing shortcoming of statically typed functional languages is that type checking does not rule out pattern-matching failures (run-time match exceptions). Refinement types distinguish different values of datatypes; if a program annotated with refinements passes type checking, pattern-matching failures become impossible. Unfortunately, refinement is a monolithic property of a type, exacerbating the difficulty of adding refinement types to nontrivial programs. Gradual typing has explored how to incrementally move between static typing and dynamic typing. We develop a type system of gradual sums that combines refinement with imprecision. Then, we develop a bidirectional version of the type system, which rules out excessive imprecision, and give a type-directed translation to a target language with explicit casts. We prove that the static sublanguage cannot have match failures, that a well-typed program remains well-typed if its type annotations are made less precise, and that making annotations less precise causes target programs to fail later. Several of these results correspond to criteria for gradual typing given by Siek et al. (2015).

==> fig-diagram-talk-intro.tex <==
\def\Highlight#1#2{\ifnum\FigVersion=#1
  \Rtexthilite{2}{yellow!50}{#2}%
  \else
  #2
\fi}

\def\RfadeContingent#1#2{\ifnum\FigVersion=1
  \Rfade{#1}{#2}%
\else
  {#2}
\fi}

\def\Metatheory#1#2{\ifnum\FigVersion=4
   \text{#2}
\else
   {\ifnum\FigVersion=5
   \Rfade{#1}{\text{#2}}
\else
   \relax
\fi}
\fi}

\mathligsoff
$~\hspace*{-10pt}$
\begin{tikzpicture}
  [auto, node distance=5ex, >=stealth, %
   descr/.style= {fill=white, inner sep=2.5pt, anchor=center}
  ]
  \node (bidir) {$e \synchk A$};
%

  \draw [->] ($(bidir.north)+(-2.5ex,0.0ex)$) arc (45:315:2.3ex); %
  
  \node[below of=bidir, node distance=5ex, left=2ex] (varyinglabel) {\fontsz{8pt}{\tabularenv{varying \\ precision \\ \Metatheory{5}{Thm.\ 4}}}};

 \node[above of=bidir, node distance=6.5ex] {\RfadeContingent{1}{\fontsz{9pt}{\tabularenv{Source \\ bidirectional \\ type system}}}};

  \node [right of=bidir, node distance=15ex] (assignment) {$e : A$};
    \draw [->] ($(bidir.east)+(0pt,3pt)$)
    -- node[above] {\fontsz{9.1pt}{\Metatheory{2}{Thm.\ 2}}}
    ($(assignment.west)+(0pt,3pt)$);
    \draw [<-] ($(bidir.east)+(0pt,-3pt)$)
    -- node[below] {\fontsz{9.1pt}{\Metatheory{2}{Thm.\ 3}}}
    ($(assignment.west)+(0pt,-3pt)$);

  \node [right of=assignment, node distance=15ex] (targetleft) {$M : T$};
    \draw [right hook->] (assignment)
    -- node[below] {\RfadeContingent{3}{\fontsz{9pt}{\tabularenv{type-directed \\ translation}}}}
    node[above] {\fontsz{9.1pt}{\Metatheory{3}{Thm.\ 9}}}
    (targetleft);

 \node[above of=assignment, node distance=5ex] {%
   \RfadeContingent{2}{\fontsz{9pt}{\tabularenv{Source \\ type assignment \\ system}}}};


  \node [right of=targetleft, node distance=13ex] (targetright) {$M' : T$};
    \draw [|->] (targetleft)
    -- node[above] {\fontsz{9.1pt}{steps to}}
    (targetright);

    \node[below of=targetright, node distance=4ex, left=-7.5ex]
       {\fontsz{9.1pt}{\Metatheory{4}{type safety (Thms.\ 6,
           7)}}};

 \node[above of=targetleft, right=-3ex, node distance=6ex] {\RfadeContingent{3}{\fontsz{9pt}{\tabularenv{Target type system \\ with run-time casts}}}};

  \node [below of=bidir, node distance=10ex] (bidirstatic) {$\eS \synchk \AS$};
    \draw [->] ($(bidir.south)+(3pt,0pt)$)
    -- node[left] {}
    ($(bidirstatic.north)+(3pt,0pt)$);
    \draw [<-] ($(bidir.south)+(-3pt,-0pt)$)
    -- node[right] {\fontsz{9.1pt}{\;\;\Metatheory{6}{Thm.\ 5}}}
    ($(bidirstatic.north)+(-3pt,0pt)$);

    \node[below of=bidirstatic, node distance=5ex, right=-6ex] {\RfadeContingent{4}{\fontsz{10pt}{\tabularenvl{%
          static sublanguage
          \\
          \textbf{(no $\mathligson +? \mathligsoff$)}
        }}}};

  \node [below of=targetleft, node distance=10ex] (targetleftstatic)
    {$M : T$}
    ;
    \draw [right hook->] (bidirstatic)
    -- node[below] {}
    (targetleftstatic);

    \node[below of=targetleftstatic, node distance=4ex]
    {\RfadeContingent{5}{\fontsz{10pt}{\tabularenv{matchfail-free}}}};

  \node [right of=targetleftstatic, node distance=13ex] (targetrightstatic) {$M' : T$};
    \draw [|->] (targetleftstatic)
    -- node[above] {}
    (targetrightstatic);

    \node[below of=targetrightstatic, node distance=4ex]
    {\RfadeContingent{6}{\fontsz{10pt}{\tabularenv{matchfail-free}}}};
\end{tikzpicture}

\mathligson
\ifnum\FigVersion=2
%
%
%
%
%
%
%
\fi


==> fig-diagram-talk-meta.tex <==
\def\Highlight#1#2{\ifnum\FigVersion=#1
  \Rtexthilite{2}{yellow!50}{#2}%
  \else
  #2
\fi}

\def\RfadeContingent#1#2{\ifnum\FigVersion=1
  \Rfade{#1}{#2}%
\else
  {#2}
\fi}

\def\Metatheory#1#2{\ifnum\FigVersion=4
   \text{#2}
\else
   {\ifnum\FigVersion=5
   \Rfade{#1}{\text{#2}}
\else
   \relax
\fi}
\fi}

\mathligsoff
$~\hspace*{-10pt}$
\begin{tikzpicture}
  [auto, node distance=5ex, >=stealth, %
   descr/.style= {fill=white, inner sep=2.5pt, anchor=center}
  ]
  \node (bidir) {$e \synchk A$};
%

  \draw [->] ($(bidir.north)+(-2.5ex,0.0ex)$) arc (45:315:2.3ex); %
  
  \node[below of=bidir, node distance=5ex, left=2ex] (varyinglabel) {\fontsz{8pt}{\tabularenv{varying \\ precision \\ \Metatheory{5}{Thm.\ 4}}}};

 \node[above of=bidir, node distance=6.5ex] {\Highlight{2}{\fontsz{9pt}{\tabularenv{Source \\ bidirectional \\ type system \\ \Metatheory{1}{Thm.\ 1}}}}};

  \node [right of=bidir, node distance=15ex] (assignment) {$e : A$};
    \draw [->] ($(bidir.east)+(0pt,3pt)$)
    -- node[above] {\fontsz{9.1pt}{\Metatheory{2}{Thm.\ 2}}}
    ($(assignment.west)+(0pt,3pt)$);
    \draw [<-] ($(bidir.east)+(0pt,-3pt)$)
    -- node[below] {\fontsz{9.1pt}{\Metatheory{2}{Thm.\ 3}}}
    ($(assignment.west)+(0pt,-3pt)$);

  \node [right of=assignment, node distance=15ex] (targetleft) {$M : T$};
    \draw [right hook->] (assignment)
    -- node[below] {\Highlight{3}{\fontsz{9pt}{\tabularenv{type-directed \\ translation}}}}
    node[above] {\fontsz{9.1pt}{\Metatheory{3}{Thm.\ 9}}}
    (targetleft);

 \node[above of=assignment, node distance=5ex] {%
   \Highlight{1}{\fontsz{9pt}{\tabularenv{Source \\ type assignment \\ system}}}};


  \node [right of=targetleft, node distance=13ex] (targetright) {$M' : T$};
    \draw [|->] (targetleft)
    -- node[above] {\fontsz{9.1pt}{steps to}}
    (targetright);

    \node[below of=targetright, node distance=4ex, left=-7.5ex]
       {\fontsz{9.1pt}{\Metatheory{4}{type safety (Thms.\ 6,7)}}};

 \node[above of=targetleft, right=-3ex, node distance=6ex] {\Highlight{3}{\fontsz{9pt}{\tabularenv{Target type system \\ with run-time casts}}}};

  \node [below of=bidir, node distance=10ex] (bidirstatic) {$\eS \synchk \AS$};
    \draw [->] ($(bidir.south)+(3pt,0pt)$)
    -- node[left] {}
    ($(bidirstatic.north)+(3pt,0pt)$);
    \draw [<-] ($(bidir.south)+(-3pt,-0pt)$)
    -- node[right] {\fontsz{9.1pt}{\;\;\Metatheory{6}{Thm.\ 5}}}
    ($(bidirstatic.north)+(-3pt,0pt)$);

    \node[below of=bidirstatic, node distance=5ex, right=-6ex] {\fontsz{10pt}{\tabularenvl{%
          static sublanguage
          \\
          \textbf{(no $\mathligson +? \mathligsoff$)}
        }}};

  \node [below of=targetleft, node distance=10ex] (targetleftstatic)
    {$M : T$}
    ;
    \draw [right hook->] (bidirstatic)
    -- node[below] {}
    (targetleftstatic);

    \node[below of=targetleftstatic, node distance=4ex]
    {\fontsz{10pt}{\tabularenv{matchfail-free \\ \Metatheory{7}{Thm.\ 10}}}};

  \node [right of=targetleftstatic, node distance=13ex] (targetrightstatic) {$M' : T$};
    \draw [|->] (targetleftstatic)
    -- node[above] {}
    (targetrightstatic);

    \node[below of=targetrightstatic, node distance=4ex]
    {\fontsz{10pt}{\tabularenv{matchfail-free \\ \Metatheory{8}{Thm.\ 8}}}};
\end{tikzpicture}

\mathligson
\ifnum\FigVersion=2
%
%
%
%
%
%
%
\fi


==> fig-diagram-talk.tex <==
\def\Highlight#1#2{\ifnum\FigVersion=#1
  \Rtexthilite{2}{yellow!50}{#2}%
  \else
  #2
\fi}

\def\RfadeContingent#1#2{\ifnum\FigVersion=1
  \Rfade{#1}{#2}%
\else
  {#2}
\fi}

\def\Metatheory#1#2{\ifnum\FigVersion=4
   \text{#2}
\else
   {\ifnum\FigVersion=5
   \Rfade{#1}{\text{#2}}
\else
   \relax
\fi}
\fi}

\mathligsoff
$~\hspace*{-10pt}$
\begin{tikzpicture}
  [auto, node distance=5ex, >=stealth, %
   descr/.style= {fill=white, inner sep=2.5pt, anchor=center}
  ]
  \node (bidir) {$e \synchk A$};
%

  \draw [->] ($(bidir.north)+(-2.5ex,0.0ex)$) arc (45:315:2.3ex); %
  
  \node[below of=bidir, node distance=5ex, left=2ex] (varyinglabel) {\fontsz{8pt}{\tabularenv{varying \\ precision \\ \Metatheory{5}{Thm.\ 4}}}};

 \node[above of=bidir, node distance=6.5ex] {\Highlight{2}{\fontsz{9pt}{\tabularenv{Source \\ bidirectional \\ type system}}}};

  \node [right of=bidir, node distance=15ex] (assignment) {$e : A$};
    \draw [->] ($(bidir.east)+(0pt,3pt)$)
    -- node[above] {\fontsz{9.1pt}{\Metatheory{2}{Thm.\ 2}}}
    ($(assignment.west)+(0pt,3pt)$);
    \draw [<-] ($(bidir.east)+(0pt,-3pt)$)
    -- node[below] {\fontsz{9.1pt}{\Metatheory{2}{Thm.\ 3}}}
    ($(assignment.west)+(0pt,-3pt)$);

  \node [right of=assignment, node distance=15ex] (targetleft) {$M : T$};
    \draw [right hook->] (assignment)
    -- node[below] {\Highlight{3}{\fontsz{9pt}{\tabularenv{type-directed \\ translation}}}}
    node[above] {\fontsz{9.1pt}{\Metatheory{3}{Thm.\ 9}}}
    (targetleft);

 \node[above of=assignment, node distance=5ex] {%
   \Highlight{1}{\fontsz{9pt}{\tabularenv{Source \\ type assignment \\ system}}}};


  \node [right of=targetleft, node distance=13ex] (targetright) {$M' : T$};
    \draw [|->] (targetleft)
    -- node[above] {\fontsz{9.1pt}{steps to}}
    (targetright);

    \node[below of=targetright, node distance=4ex, left=-7.5ex]
       {\fontsz{9.1pt}{\Metatheory{4}{type safety (Thms.\ 6,
           7)}}};

 \node[above of=targetleft, right=-3ex, node distance=6ex] {\Highlight{3}{\fontsz{9pt}{\tabularenv{Target type system \\ with run-time casts}}}};

  \node [below of=bidir, node distance=10ex] (bidirstatic) {$\eS \synchk \AS$};
    \draw [->] ($(bidir.south)+(3pt,0pt)$)
    -- node[left] {}
    ($(bidirstatic.north)+(3pt,0pt)$);
    \draw [<-] ($(bidir.south)+(-3pt,-0pt)$)
    -- node[right] {\fontsz{9.1pt}{\;\;\Metatheory{6}{Thm.\ 5}}}
    ($(bidirstatic.north)+(-3pt,0pt)$);

    \node[below of=bidirstatic, node distance=5ex, right=-6ex] {\fontsz{10pt}{\tabularenvl{%
          static sublanguage
          \\
          \textbf{(no $\mathligson +? \mathligsoff$)}
        }}};

  \node [below of=targetleft, node distance=10ex] (targetleftstatic)
    {$M : T$}
    ;
    \draw [right hook->] (bidirstatic)
    -- node[below] {}
    (targetleftstatic);

    \node[below of=targetleftstatic, node distance=4ex]
    {\fontsz{10pt}{\tabularenv{matchfail-free \\ \Metatheory{7}{Thm.\ 10}}}};

  \node [right of=targetleftstatic, node distance=13ex] (targetrightstatic) {$M' : T$};
    \draw [|->] (targetleftstatic)
    -- node[above] {}
    (targetrightstatic);

    \node[below of=targetrightstatic, node distance=4ex]
    {\fontsz{10pt}{\tabularenv{matchfail-free \\ \Metatheory{8}{Thm.\ 8}}}};
\end{tikzpicture}

\mathligson
\ifnum\FigVersion=2
%
%
%
%
%
%
%
\fi

